DriveStack-VLA: Render-Teacher Alignment for BEV-Based DeepStack Vision-Language-Action Model

Vision-Language-Action driving models convert a pretrained Vision-Language Model into a driving policy, allowing them to use world knowledge and follow language guidances. However, existing VLA driving models still lack driving-oriented spatial intelligence: their policies are mainly grounded on perspective image tokens and language priors, while precise motion planning requires metric geometry, top-down scene structure, and attention to safety-critical perceptual cues. This limitation makes current models vulnerable to weak visual geometry modeling and perceptual coverage in expert demonstrations. In this paper, we present DriveStack-VLA, a framework built upon a large VLM backbone. To strengthen the spatial grounding of VLA driving, we develop dual visual modeling components. We inject a Bird-Eye-View representation into the Large Language Model decoder through a DeepStack-style connection, and propose Render-Teacher Alignment to align the perceptual focus of real images with that of rasterized images. Furthermore, to bridge the gap in multimodal trajectory selection, we introduce a head-based self-critique module that ranks sampled trajectories and conditionally refines the best one. DriveStack-VLA achieves 91.6 PDMS on NAVSIMv1, 91.0 EPDMS on NAVSIMv2 (with the human penalty filter enabled), and a driving score of 79.49 with a success rate of 56.36\% on the closed-loop Bench2Drive. More visualizations are available on our project page: https://anonymous.4open.science/w/drivestack-vla/.

==> ieeeconf_2/Raster_Vla/figures/fig4_trajvis.tex <==
\begin{figure}[tb]
      \centering
       % 1. 压减图片与 Caption 之间的距离
      \setlength{\abovecaptionskip}{4pt} 
      % 2. 压减 Caption 与下方正文之间的距离
      \setlength{\belowcaptionskip}{-14pt}
      \includegraphics[width=\linewidth]{ieeeconf_2/Raster_Vla/figures/fig/fig-4_trajectory_comparison_20260305.pdf}
      % \vspace{-1pt}
      \captionsetup{font={small}}
      \caption{Qualitative comparison with the VLM backbone following SFT.}
      \label{fig:trajvis}
\end{figure}

